Can Vehicle Motion Planning Generalize to Realistic Long-tail Scenarios?

Real-world autonomous driving systems must make safe decisions in the face of rare and diverse traffic scenarios. Current state-of-the-art planners are mostly evaluated on real-world datasets like nuScenes (open-loop) or nuPlan (closed-loop). In particular, nuPlan seems to be an expressive evaluation method since it is based on real-world data and closed-loop, yet it mostly covers basic driving scenarios. This makes it difficult to judge a planner's capabilities to generalize to rarely-seen situations. Therefore, we propose a novel closed-loop benchmark interPlan containing several edge cases and challenging driving scenarios. We assess existing state-of-the-art planners on our benchmark and show that neither rule-based nor learning-based planners can safely navigate the interPlan scenarios. A recently evolving direction is the usage of foundation models like large language models (LLM) to handle generalization. We evaluate an LLM-only planner and introduce a novel hybrid planner that combines an LLM-based behavior planner with a rule-based motion planner that achieves state-of-the-art performance on our benchmark.

==> tab/tab3_motion_vs_behavior.tex <==
\begin{table}[t!]
    \vspace{-0.0cm}
    \centering
    \setlength{\tabcolsep}{10pt}
    \resizebox{0.4\textwidth}{!}{
        \begin{tabular}{rlrrrrrrr}
            \toprule
            \multirow{1}{*}{\textbf{Method}} & \textbf{Output} & {\textbf{interPlan-Score} $\uparrow$}\\
            \midrule
            \texttt{LLama-7B} & Waypoints & ? \\
            \texttt{LLama-13B} & Waypoints & ? \\
            \texttt{GPT-3.5} & Waypoints & ? \\
            \texttt{GPT-4} & Waypoints & ? \\
            \midrule
            \texttt{LLama-7B} & Behavior & ? \\
            \texttt{LLama-13B} & Behavior & ? \\
            \texttt{GPT-3.5} & Behavior & ? \\
            \texttt{GPT-4} & Behavior & ? \\
            \bottomrule
        \end{tabular}
    }
    \vspace{0.2cm}
    \caption{\textbf{interPlan Benchmark.} TODO}
    \label{tab:motion_vs_behavior}
    \vspace{-0.5cm}
\end{table}
